Multi-dimensional Virtual Values and Second-degree Price Discrimination

We consider a multi-dimensional screening problem of selling a product with multiple quality levels and design virtual value functions to derive conditions that imply optimality of only selling highest quality. A challenge of designing virtual values for multi-dimensional agents is that a mechanism that pointwise optimizes virtual values resulting from a general application of integration by parts is not incentive compatible, and no general methodology is known for selecting the right paths for integration by parts. We resolve this issue by first uniquely solving for paths that satisfy certain necessary conditions that the pointwise optimality of the mechanism imposes on virtual values, and then identifying distributions that ensure the resulting virtual surplus is indeed pointwise optimized by the mechanism. Our method of solving for virtual values is general, and as a second application we use it to derive conditions of optimality for selling only the grand bundle of items to an agent with additive preferences.

==> unitdemandbundlepricing.tex <==
\subsection{Bundle Pricing for General Distributions}
We can use the generality of unit-demand settings and the above result
to identify conditions under which bundle pricing is optimal for general
distributions. More precisely, notice that any problem with finite
outcome space can be converted to a unit-demand problem with
dot-product utility function by letting $\typeprelim$ and
$\sagentmech$ be vectors of dimension equal to the cardinality of the outcome
space, with $t_i$ being the value for outcome $i$. For multi-item
settings with $m$ items, the size of the outcome space is equal to
$2^m$. The input to the problem is a density function
$f(t_1,\ldots,t_k)$ over vectors of dimension $k = 2^m$. We assume \emph{free disposal}, meaning that the density of a
type is non-zero only if the valuation for each bundle is at
least as much as the value for any other subset of that bundle. The
max-ratio representation of the density function is a
$\denscor{M\!R}(t_1,\theta_2,\ldots,\theta_k)$, where $t_1$, normalized to be
at most 1, is the value for the grand bundle, and $\theta_i \leq 1$ is
the ratio of the value for the $i$-th subset, over the value of the
grand bundle. Now a bundle pricing mechanism corresponds to a
mechanism in the unit demand setting which only sells the favorite
outcome, which is the grand bundle. The theorem below follows immediately from the extension of \autoref{t:uniform-pricing-strong-amortization-general} to the case of more than two items (see \autoref{a:mitems}).

\begin{theorem}
Bundle pricing is optimal if the max-ratio representation of the density function is MR-log-supermodular for which the strong amortization of the favorite item projection is monotone.
\end{theorem} 

A density function is MR-log-supermodular if its max-ratio representation $\denscor{M\!R}$ is log-supermodular, that is, for any two vectors $(t_1,\theta_2,\ldots,\theta_k)$ and $(t'_1,\theta'_2,\ldots,\theta'_k)$,
\begin{align*}
&\hspace{-6.8ex}\denscor{M\!R}(t_1,\ldots,\theta_k) \cdot \denscor{M\!R}(t'_1,\ldots,\theta'_k)\\& \leq \denscor{M\!R}(\min(t_1,t'_1),\ldots,\min(\theta_k,\theta'_k)) \cdot \denscor{M\!R}(\max(t_1,t'_1),\ldots,\max(\theta_k,\theta'_k)).
\end{align*} 

==> unitdemandonlyif.tex <==
\subsection{Necessary Conditions for Optimality of Uniform Pricing}
We now provide a partial converse to \autoref{t:uniform-pricing-strong-amortization-general}  by specifying conditions under which uniform pricing is not revenue optimal. The proof follows the approach of \citet{Tha04} in showing that uniform pricing is not optimal for the uniform independent distribution on $[5,6]$. Under the conditions of the theorem, the best uniform pricing mechanism can be improved by adding a lottery with slightly lower price, that offers each item with probability a half. The proof is deferred to \autoref{a:missing}.

\begin{theorem}
Uniform pricing is not revenue optimal if for any price $t_1$ that satisfies the first order condition of optimizing revenue $t_1( 1- \sdpdist(t_1))$,
\begin{align*}
t_1 - \frac{1- \sdpdist(t_1)}{\sdpdens(t_1) }&=  0 \intertext{the tradeoff between more sales and the loss of revenue from lowering the price as a result of adding a lottery to the menu is positive }
t_1 - 2\frac{\int_{t'_1=t_1}^1 f(t'_1,t'_1) \; \dd t'_1} {f(t_1,t_1)} &>0.
\end{align*}
\label{thm:ironedunit-general-onlyif}
\end{theorem}
